Applying Quantum Autoencoders for Time Series Anomaly Detection

Anomaly detection is an important problem with applications in various domains such as fraud detection, pattern recognition or medical diagnosis. Several algorithms have been introduced using classical computing approaches. However, using quantum computing for solving anomaly detection problems in time series data is a widely unexplored research field. This paper explores the application of quantum autoencoders to time series anomaly detection. We investigate two primary techniques for classifying anomalies: (1) Analyzing the reconstruction error generated by the quantum autoencoder and (2) latent representation analysis. Our simulated experimental results, conducted across various ansaetze, demonstrate that quantum autoencoders consistently outperform classical deep learning-based autoencoders across multiple datasets. Specifically, quantum autoencoders achieve superior anomaly detection performance while utilizing 60-230 times fewer parameters and requiring five times fewer training iterations. In addition, we implement our quantum encoder on real quantum hardware. Our experimental results demonstrate that quantum autoencoders achieve anomaly detection performance on par with their simulated counterparts.

==> assets/graphs/combined_qae.tex <==

% \scalebox{0.72}{
\Qcircuit @C=1.0em @R=0.2em @!R { \\
	 	\nghost{{0} :  } & \lstick{{0} :  } & \multigate{6}{|\phi(\vec{x})\rangle\,}_<<<{} & \multigate{6}{\mathrm{Encoder}\,}_<<<{} \barrier[0em]{8} & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{1} :  } & \lstick{{1} :  } & \ghost{|\psi\rangle\,}_<<<{} & \ghost{\mathrm{Encoder}\,}_<<<{} & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{2} :  } & \lstick{{2} :  } & \ghost{|\psi\rangle\,}_<<<{} & \ghost{\mathrm{Encoder}\,}_<<<{} & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{3} :  } & \lstick{{3} :  } & \ghost{|\psi\rangle\,}_<<<{} & \ghost{\mathrm{Encoder}\,}_<<<{} & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{4} :  } & \lstick{{4} :  } & \ghost{|\psi\rangle\,}_<<<{} & \ghost{\mathrm{Encoder}\,}_<<<{} & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{5} :  } & \lstick{{5} :  } & \ghost{|\psi\rangle\,}_<<<{} & \ghost{\mathrm{Encoder}\,}_<<<{} & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{6} :  } & \lstick{{6} :  } & \ghost{|\psi\rangle\,}_<<<{} & \ghost{\mathrm{Encoder}\,}_<<<{} & \qw & \qw & \qswap \qwx[1] & \qw & \qw & \qw & \qw\\
	 	\nghost{{7} :  } & \lstick{{7} :  } & \qw & \qw & \qw & \qw & \qswap & \qw & \qw & \qw & \qw\\
	 	\nghost{{8} :  } & \lstick{{8} :  } & \qw & \qw & \qw & \gate{\mathrm{H}} & \ctrl{-1} & \gate{\mathrm{H}} & \meter & \qw & \qw\\
	 	\nghost{\mathrm{{c} :  }} & \lstick{\mathrm{{c} :  }} & \lstick{/_{_{1}}} \cw & \cw & \cw & \cw & \cw & \cw & \dstick{_{_{\hspace{0.0em}0}}} \cw \ar @{<=} [-1,0] & \cw & \cw\\
\\ }
% }

% \scalebox{2}{

\Qcircuit @C=1.0em @R=1.0em @!R { \\
	 	\nghost{{q}_{0} :  } & \lstick{{q}_{0} :  } & \multigate{6}{|\phi(\vec{x})\rangle\,}_<<<{} & \multigate{6}{\mathrm{Encoder}\,}_<<<{} & \qw & \multigate{6}{\mathrm{Encoder^\dag}\,}_<<<{} \barrier[0em]{8} & \qw & \meter & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{q}_{1} :  } & \lstick{{q}_{} :  } & \ghost{|\psi\rangle\,}_<<<{} & \ghost{\mathrm{Encoder}\,}_<<<{} & \qw & \ghost{\mathrm{Encoder^\dag}\,}_<<<{} & \qw & \qw & \meter & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{q}_{2} :  } & \lstick{{q}_{} :  } & \ghost{|\psi\rangle\,}_<<<{} & \ghost{\mathrm{Encoder}\,}_<<<{} & \qw & \ghost{\mathrm{Encoder^\dag}\,}_<<<{} & \qw & \qw & \qw & \meter & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{q}_{3} :  } & \lstick{{q}_{} :  } & \ghost{|\psi\rangle\,}_<<<{} & \ghost{\mathrm{Encoder}\,}_<<<{} & \qw & \ghost{\mathrm{Encoder^\dag}\,}_<<<{} & \qw & \qw & \qw & \qw & \meter & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{q}_{4} :  } & \lstick{{q}_{} :  } & \ghost{|\psi\rangle\,}_<<<{} & \ghost{\mathrm{Encoder}\,}_<<<{} & \qw & \ghost{\mathrm{Encoder^\dag}\,}_<<<{} & \qw & \qw & \qw & \qw & \qw & \meter & \qw & \qw & \qw & \qw\\
	 	\nghost{{q}_{5} :  } & \lstick{{q}_{} :  } & \ghost{|\psi\rangle\,}_<<<{} & \ghost{\mathrm{Encoder}\,}_<<<{} & \qw & \ghost{\mathrm{Encoder^\dag}\,}_<<<{} & \qw & \qw & \qw & \qw & \qw & \qw & \meter & \qw & \qw & \qw\\
	 	\nghost{{q}_{6} :  } & \lstick{{q}_{} :  } & \ghost{|\psi\rangle\,}_<<<{} & \ghost{\mathrm{Encoder}\,}_<<<{} & \gate{\mathrm{\left|0\right\rangle}} & \ghost{\mathrm{Encoder^\dag}\,}_<<<{6} & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \meter & \qw & \qw\\
            \nghost{{q}_{7} :  } & \lstick{{q}_{} :  } & \qw  & \qw & \qw & \qw  & \qw & \qw & \qw & \qw & \qw & \qw & \qw  & \qw & \qw & \qw\\
            \nghost{{q}_{7} :  } & \lstick{{q}_{} :  } & \qw  & \qw & \qw & \qw  & \qw & \qw & \qw & \qw & \qw & \qw & \qw  & \qw & \qw & \qw\\
	 	\nghost{\mathrm{{meas} :  }} & \lstick{\mathrm{{meas} :  }} & \lstick{/_{_{7}}} \cw & \cw & \cw & \cw & \cw & \dstick{_{_{\hspace{0.0em}0}}} \cw \ar @{<=} [-9,0] & \dstick{_{_{\hspace{0.0em}1}}} \cw \ar @{<=} [-8,0] & \dstick{_{_{\hspace{0.0em}2}}} \cw \ar @{<=} [-7,0] & \dstick{_{_{\hspace{0.0em}3}}} \cw \ar @{<=} [-6,0] & \dstick{_{_{\hspace{0.0em}4}}} \cw \ar @{<=} [-5,0] & \dstick{_{_{\hspace{0.0em}5}}} \cw \ar @{<=} [-4,0] & \dstick{_{_{\hspace{0.0em}6}}} \cw \ar @{<=} [-3,0] & \cw & \cw\\
\\ }
% }


==> parts/problem-statement.tex <==

Time series anomaly detection is a challenging problem with broad applications spanning domains such as finance, healthcare, industrial monitoring, cybersecurity, and more. Its primary objective involves identifying atypical patterns or behaviors within sequentially ordered data points comprising a time series. The temporal aspect of time series data allows for the observation of dynamic changes over time.
 \begin{figure*}
    \centering
    \input{assets/graphs/overview}
    \caption{The high level methodology employed for anomaly detection in this study encompasses a systematic approach, beginning with data preprocessing. Subsequently, the quantum state preparation procedure is performed, followed by applying the chosen autoencoding ansatz. Upon completion of these computational phases, the resultant data is subjected to postprocessing procedures and final anomaly classification. The notations CPU and QPU delineate between actions executed on classical computing architectures (CPU) and those performed on quantum hardware platforms (QPU).}
    \label{fig:MethodologyOverview}
\end{figure*}
The intricacy of time series anomaly detection arises from the need to identify subtle deviations or rare occurrences within the underlying normal patterns. Anomalies can take various forms, including abrupt spikes, sharp declines, fluctuations, or irregular trends. Detecting these anomalies is crucial for identifying potential faults, threats, or abnormal events that may have severe consequences if left undetected. The complexity of the anomaly detection task is influenced by several factors, including the heterogeneous and complex nature of anomalies in real-world data, the presence of inherent noise or uncertainty in time series measurements, and the class imbalance between normal and anomalous instances. Additionally, the concept of anomalies is contextual and domain-specific, varying based on the specific applications. An additional challenge arises from the fact that training data usually contains only normal events, leaving anomalies as instances that deviate from the expected patterns. Consequently, leveraging a priori knowledge for training machine learning-based detection methods becomes impractical due to the subtle nature of anomalous data and their diverse manifestations. Furthermore, the scarcity of anomaly data increases the difficulty of obtaining effective anomaly detection models. To address these challenges, powerful methods are required to learn representations of normal, non-anomalous data, which often contain complex dependencies and large amounts of data to learn from. Quantum computing shows promise in this regard, excelling in handling complex data dependencies and offering potential solutions to improve anomaly detection tasks. Furthermore, data volume is steadily growing and the need of processing ever larger amount of data is imminent and is an advantage of quantum computing over traditional approaches with it's capacity to process larger amount of data more efficiently.

